Utopia: Fast and Efficient Address Translation via Hybrid Restrictive & Flexible Virtual-to-Physical Address Mappings

Conventional virtual memory (VM) frameworks enable a virtual address to flexibly map to any physical address. This flexibility necessitates large data structures to store virtual-to-physical mappings, which leads to high address translation latency and large translation-induced interference in the memory hierarchy. On the other hand, restricting the address mapping so that a virtual address can only map to a specific set of physical addresses can significantly reduce address translation overheads by using compact and efficient translation structures. However, restricting the address mapping flexibility across the entire main memory severely limits data sharing across different processes and increases data accesses to the swap space of the storage device, even in the presence of free memory. We propose Utopia, a new hybrid virtual-to-physical address mapping scheme that allows both flexible and restrictive hash-based address mapping schemes to harmoniously co-exist in the system. The key idea of Utopia is to manage physical memory using two types of physical memory segments: restrictive and flexible segments. A restrictive segment uses a restrictive, hash-based address mapping scheme that maps virtual addresses to only a specific set of physical addresses and enables faster address translation using compact translation structures. A flexible segment employs the conventional fully-flexible address mapping scheme. By mapping data to a restrictive segment, Utopia enables faster address translation with lower translation-induced interference. Utopia improves performance by 24% in a single-core system over the baseline system, whereas the best prior state-of-the-art contiguity-aware translation scheme improves performance by 13%.

==> commands_v2.tex <==
\usepackage{xspace}
\usepackage{color}
\usepackage{listings}
\usepackage{xcolor}

%for commenting%
\definecolor{darkspringgreen}{rgb}{0.09, 0.45, 0.27}
\definecolor{denim}{rgb}{0.08, 0.38, 0.74}
\definecolor{darkolivegreen}{rgb}{0.33, 0.42, 0.18}
\definecolor{tangerine}{rgb}{0.95, 0.52, 0.0}
\definecolor{mahogany}{rgb}{0.75, 0.25, 0.0}

\newcommand{\shellcmd}[1]{\indent\indent\texttt{\footnotesize\$ #1}}

\definecolor{uglyyellow}{rgb}{0.99, 0.93, 0.0}
\definecolor{nbs}{rgb}{0.35, 0.31, 0.81}
\newcommand{\nb}[1]{\textcolor{black}{#1}}
\newcommand{\numplaceholder}[1]{\textcolor{red}{#1}}
\newcommand{\nbc}[1]{\todo[size=\scriptsize, linecolor=black, bordercolor=black, backgroundcolor=white]{\textcolor{nbs}{\textbf{@nb:} #1}}}
% \newcommand{\nbc}[1]{{\textcolor{nbs}{\colorbox{uglyyellow}{\textbf{{[@nb:}}} \colorbox{uglyyellow}{{#1}\textbf{]}}}}}
\definecolor{darkred}{rgb}{0.75, 0.1, 0.1}
\newcommand{\dbb}[1]{\textcolor{black}{#1}}
\newcommand{\dbbc}[1]{\todo[size=\scriptsize, linecolor=black, bordercolor=black, backgroundcolor=white]{\textcolor{darkred}{\textbf{@dbb:} #1}}}

\newcommand{\revD}[1]{\textcolor{purple}{#1}}
\newcommand{\revA}[1]{\textcolor{green}{#1}}
\newcommand\hm[1]{{\color{black}{#1}}}
\newcommand\hmc[1]{{\color{darkolivegreen}{\fbox{\textsc{\textbf{Harun:}}} \textit{#1}}}}


%%%%revision



\newcommand\konkanello[1]{\textcolor{blue}{#1}}
\newcommand{\hong}[1]{\textcolor{pink}{#1}}






% \newcolumntype{Y}{>{\centering\arraybackslash}X}
\usepackage{tikz}
% \newcommand{\circlednumber}[1]{\raisebox{0.5pt}{\protect%
%   \tikz[baseline=(myanchor.base)]{
%   \node[circle,fill=.,inner sep=1pt] (myanchor) {\color{-.}\footnotesize #1};}%
% }}
\newcommand{\circlednumber}[1]{\tikz[baseline=(char.base)]{
           \node[shape=circle,draw,inner sep=0pt,fill=black, text=white] (char) {#1};}}


\newcommand{\squishlist}{
 \begin{list}{$\circ$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{0pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} } }

\newenvironment{squishenum}
{\begin{enumerate}[leftmargin=*]
  \setlength{\itemsep}{0em}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
  \setlength{\topsep}{3pt}
  \setlength{\partopsep}{0pt}}
{\end{enumerate}}

\newcommand{\squishend}{
  \end{list}  }
  
  
  


\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,fill,inner sep=0.5pt] (char) {\textcolor{white}{#1}};}}
\newcommand*\circledwhite[1]{\tikz[baseline=(char.base)]{\node[shape=circle, inner sep=0.5pt, draw=black, fill=white, text=black] (char) {#1};}}


% \newcommand\todo[1]{\noindent{\color{magenta} {\fbox{\bf{TODO: }}\it"#1"}}}


\usepackage[colorinlistoftodos,prependcaption,textsize=scriptsize]{todonotes}

% \setlength {\marginparwidth}{1cm}
% \usepackage[colorinlistoftodos,prependcaption,textsize=scriptsize]{todonotes} % For margin notes
% \usepackage{marginnote} 
% \let\marginpar\marginnote
% \setlength{\marginparwidth}{0.5in}

% \usepackage[colorinlistoftodos,prependcaption,textsize=scriptsize]{todonotes}
% %%%%%%%%%%%% Extend the margin for todo-notes %%%%%%%%%%%% 
%     \paperwidth=\dimexpr \paperwidth + 4cm\relax
%     \oddsidemargin=\dimexpr\oddsidemargin + 2cm\relax
%     \evensidemargin=\dimexpr\evensidemargin + 2cm\relax
%     \marginparwidth=\dimexpr \marginparwidth + 2cm\relax





% \setlength{\marginparwidth}{1.3cm}

\usepackage[bottom]{footmisc}
\usepackage{dblfloatfix}
\usepackage{array}
 \usepackage{booktabs}
% \renewcommand{\subsectionautorefname}{Section}
% \renewcommand{\subsubsectionautorefname}{Section}

\newcommand\head[1]{{\noindent\textbf{#1}.}}
% \documentclass[usenames,dvipsnames]{beamer}
\definecolor{ufogreen}{rgb}{0.1, 0.6, 0.4}
\definecolor{ufogreen}{rgb}{0.1, 0.6, 0.4}

\newcommand\new[1]{{\color{blue}{#1}}}
\newcommand\kanel[1]{{\color{magenta}{#1}}}


\newcommand{\system}{Victima\xspace}
\newcommand{\speedupoverbaseline}{7.4} % for referencing sections
\newcommand{\speedupoverpomtlb}{5.1} % for referencing sections
\newcommand{\speedupoverbaselinevirt}{20.4} % for referencing sections
\newcommand{\speedupoverispvirt}{2.4} % for referencing sections
\newcommand{\speedupoverpomtlbvirt}{12.3} % for referencing sections
\newcommand{\latencyoverbaselinenative}{33.2}
\newcommand{\latencyoverbaselinevirt}{40.4}
\newcommand{\latencyoverpomtlbvirt}{73.9}
\newcommand{\latenctoverispvirt}{46.4}
\newcommand{\area}{0.02} % for referencing sections
\newcommand{\power}{0.04} % for referencing sections
\newcommand{\tlbreusezero}{38.7}
\newcommand{\ptwreductionoverbaseline}{53.3}
\newcommand{\ptwreductionoverbaselinemax}{92.6}

\usepackage{listings}
\usepackage{xcolor}
\usepackage[T1]{fontenc} % Needed for correct font encoding
\usepackage{zi4} % Load the Inconsolata font package
\usepackage{caption} % Load the caption package
\usepackage{float} % Load the float package

\lstdefinestyle{custompseudocode}{
  belowcaptionskip=1\baselineskip,
  breaklines=true,
  xleftmargin=\parindent,
  language=Python,
  showstringspaces=false,
  basicstyle=\small\ttfamily,
  keywordstyle=\bfseries\color{green!40!black},
  commentstyle=\itshape\color{purple},
  stringstyle=\color{orange},
  numbers=left,
  numberstyle=\scriptsize\color{black},
  numbersep=8pt,
  morekeywords={function}, % Added function keyword
  keywordstyle=[2]\bfseries, % Added new keyword class with bold style
  escapeinside={*@}{@*}, % Added escape sequence
  xleftmargin=2em, xrightmargin=0em, 
}
\DeclareCaptionFormat{listing}{% Define the caption format
  \rule{\linewidth}{0.5pt}
  \vspace{-1mm}
  \textbf{#1#2: }#3
  \vspace{-1mm}
  \rule{\linewidth}{0.5pt}
  \vspace{-7mm}
}



\captionsetup[lstlisting]{format=listing, singlelinecheck=false}



\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
\definecolor{chocolate}{rgb}{0.92, 0.41, 0.12}
\definecolor{burgundy}{rgb}{0.5, 0.0, 0.13}
\definecolor{darkmagenta}{rgb}{0.55, 0.0, 0.55}
\definecolor{darkblue}{rgb}{0.0, 0.5, 1.0}
\newcommand\konkanelloreva[1]{\textcolor{black}{#1}}
\newcommand\konkanellorevb[1]{\textcolor{black}{#1}}
\newcommand\konkanellorevc[1]{\textcolor{black}{#1}}
\newcommand\konkanellorevd[1]{\textcolor{black}{#1}}
\newcommand\konkanelloreve[1]{\textcolor{black}{#1}}





